Self-supervised Multi-future Occupancy Forecasting for Autonomous Driving

Environment prediction frameworks are critical for the safe navigation of autonomous vehicles (AVs) in dynamic settings. LiDAR-generated occupancy grid maps (L-OGMs) offer a robust bird's-eye view for the scene representation, enabling self-supervised joint scene predictions while exhibiting resilience to partial observability and perception detection failures. Prior approaches have focused on deterministic L-OGM prediction architectures within the grid cell space. While these methods have seen some success, they frequently produce unrealistic predictions and fail to capture the stochastic nature of the environment. Additionally, they do not effectively integrate additional sensor modalities present in AVs. Our proposed framework, Latent Occupancy Prediction (LOPR), performs stochastic L-OGM prediction in the latent space of a generative architecture and allows for conditioning on RGB cameras, maps, and planned trajectories. We decode predictions using either a single-step decoder, which provides high-quality predictions in real-time, or a diffusion-based batch decoder, which can further refine the decoded frames to address temporal consistency issues and reduce compression losses. Our experiments on the nuScenes and Waymo Open datasets show that all variants of our approach qualitatively and quantitatively outperform prior approaches.

==> New_Figures/fig_1.tex <==
\def\imgone{scene-0082_270}

\scalebox{0.6}{
% \hspace*{-0.58cm}
\begin{tikzpicture}
    % -- Define row/column gaps and image size --
    \def\rowgap{1.5}     % vertical spacing between rows
    \def\colgap{1.5}     % horizontal spacing between columns
    \def\imgsize{1.35cm}  % width and height for each image
    
    % -- Time intervals and frames --
    \def\timesteps{0.5, 1, 1.5, 2, 2.5, 3}
    \def\frames{4,9,14,19,24,29}

    % ----------------------------------------------------------------
    % Ground Truth row (y = 0)
    % ----------------------------------------------------------------
    \foreach \t [count=\i] in \timesteps
    {
      % Compute x-position for column i
      \pgfmathsetmacro\xpos{\colgap * \i}
      % Index from \frames
      \pgfmathsetmacro\frameindex{{\frames}[\i-1]}

      % Place Ground Truth image (thin black border)
      \node[draw=black, thin, inner sep=0pt] (gtimage\i)
          at (\xpos, 0)
          {\includegraphics[width=\imgsize,height=\imgsize]{New Figures/\imgone/fixed_gt_\frameindex.png}}; %\frameindex_gt.png

      % Label above each Ground Truth image (tiny time annotation)
      \node[font=\tiny] at (\xpos, 0.8) {\pgfmathprintnumber{\t} s};
    }

    % "Ground Truth" label anchored to the west edge of the first GT image
    \node[
      rotate=90,
      anchor=east,
      font=\tiny,
      inner sep=0pt,
      xshift=14pt,
      yshift=4pt
    ]
    at (gtimage1.west) {Ground Truth};

    % ----------------------------------------------------------------
    % Best row (y = -\rowgap)
    % ----------------------------------------------------------------
    \foreach \t [count=\i] in \timesteps
    {
      \pgfmathsetmacro\xpos{\colgap * \i}
      \pgfmathsetmacro\frameindex{{\frames}[\i-1]}

      \node[draw=black, thin, inner sep=0pt] (bestimage\i)
          at (\xpos, -\rowgap)
          {\includegraphics[width=\imgsize,height=\imgsize]{New Figures/\imgone/\frameindex_pred_1.png}};
    }

    % "IS=3.64" label for the Best row
    \node[
      rotate=90,
      anchor=east,
      font=\tiny,
      inner sep=0pt,
      xshift=8pt,
      yshift=4pt
    ]
    at (bestimage1.west) {Ours};

    % ----------------------------------------------------------------
    % Random row (y = -2*\rowgap)
    % ----------------------------------------------------------------
    \foreach \t [count=\i] in \timesteps
    {
      \pgfmathsetmacro\xpos{\colgap * \i}
      \pgfmathsetmacro\frameindex{{\frames}[\i-1]}

      \node[draw=black, thin, inner sep=0pt] (randimage\i)
          at (\xpos, -2*\rowgap)
          {\includegraphics[width=\imgsize,height=\imgsize]{New Figures/\imgone/occworld/scene-0082_241_pred_\frameindex.png}};
    }

    % "IS=5.29" label for the Random row
    \node[
      rotate=90,
      anchor=east,
      font=\tiny,
      inner sep=0pt,
      xshift=11pt,
      yshift=4pt
    ]
    at (randimage1.west) {OccWorld};

    % ----------------------------------------------------------------
    % Extra image on the right (not part of the row logic)
    % ----------------------------------------------------------------
    % \node[draw=black, thin, inner sep=0pt]
    %     (extraimage) at (11.33, -0.07)
    %     {\includegraphics[height=1.5cm]{New Figures/\imgone/CAM_FRONT_last.png}};

    % ----------------------------------------------------------------
    % Red circles and arrow
    % (Adjust coordinates/size as needed)
    % ----------------------------------------------------------------
    \draw[red, line width=1pt, opacity=0.5] (3.7, 0.20) circle (0.3cm);
    \draw[red, line width=1pt, opacity=0.5] (4.75, 0.20) circle (0.3cm);
    \draw[red, line width=1pt, opacity=0.5] (5.9, 0.20) circle (0.3cm);
    \draw[red, line width=1pt, opacity=0.5] (6.9, 0.20) circle (0.3cm);
    % \draw[red, line width=1pt, opacity=0.5] (11.11, -0.18) circle (0.3cm);
    % \draw[<-, thick, red, opacity=0.75] (9.68, 0.67) -- (9.98, 0.67);
\end{tikzpicture}   
  }

==> New_Figures/fig_2.tex <==
\def\imgone{scene-0551}

\scalebox{0.6}{
% \hspace*{-0.58cm}
\begin{tikzpicture}
    % -- Define row/column gaps and image size --
    \def\rowgap{1.5}     % vertical spacing between rows
    \def\colgap{1.5}     % horizontal spacing between columns
    \def\imgsize{1.35cm}  % width and height for each image
    
    % -- Time intervals and frames --
    \def\timesteps{0.5, 1, 1.5, 2, 2.5, 3}
    \def\frames{4,9,14,19,24,29}

    % ----------------------------------------------------------------
    % Ground Truth row (y = 0)
    % ----------------------------------------------------------------
    \foreach \t [count=\i] in \timesteps
    {
      % Compute x-position for column i
      \pgfmathsetmacro\xpos{\colgap * \i}
      % Index from \frames
      \pgfmathsetmacro\frameindex{{\frames}[\i-1]}

      % Place Ground Truth image (thin black border)
      \node[draw=black, thin, inner sep=0pt] (gtimage\i)
          at (\xpos, 0)
          {\includegraphics[width=\imgsize,height=\imgsize]{New Figures/\imgone/occworld/\imgone_1_gt_\frameindex.png}};

      % Label above each Ground Truth image (tiny time annotation)
      \node[font=\tiny] at (\xpos, 0.8) {\pgfmathprintnumber{\t} s};
    }

    % "Ground Truth" label anchored to the west edge of the first GT image
    \node[
      rotate=90,
      anchor=east,
      font=\tiny,
      inner sep=0pt,
      xshift=14pt,
      yshift=4pt
    ]
    at (gtimage1.west) {Ground Truth};

    % ----------------------------------------------------------------
    % Best row (y = -\rowgap)
    % ----------------------------------------------------------------
    \foreach \t [count=\i] in \timesteps
    {
      \pgfmathsetmacro\xpos{\colgap * \i}
      \pgfmathsetmacro\frameindex{{\frames}[\i-1]}

      \node[draw=black, thin, inner sep=0pt] (bestimage\i)
          at (\xpos, -\rowgap)
          {\includegraphics[width=\imgsize,height=\imgsize]{New Figures/\imgone/\frameindex_pred_1.png}};
    }

    % "IS=3.64" label for the Best row
    \node[
      rotate=90,
      anchor=east,
      font=\tiny,
      inner sep=0pt,
      xshift=8pt,
      yshift=4pt
    ]
    at (bestimage1.west) {Ours};

    % ----------------------------------------------------------------
    % Random row (y = -2*\rowgap)
    % ----------------------------------------------------------------
    \foreach \t [count=\i] in \timesteps
    {
      \pgfmathsetmacro\xpos{\colgap * \i}
      \pgfmathsetmacro\frameindex{{\frames}[\i-1]}

      \node[draw=black, thin, inner sep=0pt] (randimage\i)
          at (\xpos, -2*\rowgap)
          {\includegraphics[width=\imgsize,height=\imgsize]{New Figures/\imgone/occworld/\imgone_1_pred_\frameindex.png}};
    }

    % "IS=5.29" label for the Random row
    \node[
      rotate=90,
      anchor=east,
      font=\tiny,
      inner sep=0pt,
      xshift=11pt,
      yshift=4pt
    ]
    at (randimage1.west) {OccWorld};

    % ----------------------------------------------------------------
    % Extra image on the right (not part of the row logic)
    % ----------------------------------------------------------------
    % \node[draw=black, thin, inner sep=0pt]
    %     (extraimage) at (11.33, -0.07)
    %     {\includegraphics[height=1.5cm]{New Figures/\imgone/CAM_FRONT_last.png}};

    % ----------------------------------------------------------------
    % Red circles and arrow
    % (Adjust coordinates/size as needed)
    % ----------------------------------------------------------------
    \draw[orange, line width=1pt, opacity=0.5] (1.8, 0.20) circle (0.3cm);
    \draw[orange, line width=1pt, opacity=0.5] (2.75, 0.20) circle (0.3cm);
    \draw[orange, line width=1pt, opacity=0.5] (3.9, 0.20) circle (0.3cm);
    % \draw[orange, line width=1pt, opacity=0.5] (10.65, -0.18) circle (0.35cm);

    % \draw[<-, thick, orange, opacity=0.75] (9.68, 0.67) -- (9.98, 0.67);
\end{tikzpicture}   
  }

==> Tables/latent_space.tex <==
\begin{table*}[h]
    \centering
    \caption{Impact of KL regularization during representation learning on LOPR's performance in terms of reconstruction and a simplified prediction task using the NuScenes dataset. For all metrics, lower is better.}
    \tiny 
    \begin{tabular}{@{}lcccc@{}}
      \toprule
      \textbf{KL} & \textbf{OGM Recon. (IS)} & \textbf{OGM Prediction (IS)} & \textbf{Camera Recon. (MSE)} & \textbf{Map Recon. (MSE)} \\ 
      \midrule
      \num{1e-06} & 3.51 $\pm$ 0.01 & 14.85 $\pm$ 0.72 & \textbf{2.21 $\pm$ 0.04} & \textbf{0.49 $\pm$ 0.04}  \\
      \num{1.0} & \textbf{1.71 $\pm$ 0.01} & 15.90 $\pm$ 0.34 & 2.89 $\pm$ 0.07  & 0.51 $\pm$ 0.06 \\
      \num{4.0} & 1.75 $\pm$ 0.01 & \textbf{13.19 $\pm$ 0.42} & 3.12 $\pm$ 0.06 & 0.53 $\pm$ 0.07 \\
      \bottomrule
    \end{tabular}
  \label{tab:kl}
%\vspace{-2.7em} % Add some vertical spacing between the rows
\end{table*}

